On the arbitrarily long-term stability of conservative methods

We show the arbitrarily long-term stability of conservative methods for autonomous ODEs. Given a system of autonomous ODEs with conserved quantities, if the preimage of the conserved quantities possesses a bounded locally nite neighborhood, then the global error of any conservative method with the uniformly bounded displacement property is bounded for all time, when the uniform time step is taken suciently small. On nite precision machines, the global error still remains bounded and independent of time until some arbitrarily large time determined by machine precision and tolerance. The main result is proved using elementary topological properties for discretized conserved quantities which are equicontinuous. In particular, long-term stability is also shown using an averaging identity when the discretized conserved quantities do not explicitly depend on time steps. Numerical results are presented to illustrate the long-term stability result.

==> SINUM Final/CM_stability_info.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx,epstopdf}
\usepackage[caption=false]{subfig}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{On the arbitrarily long-term stability of conservative methods} 
\newcommand{\TheAuthors}{Andy T. S. Wan, and Jean-Christophe Nave}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{This work was supported by the NSERC Discovery program and the Centre de Recherches Math\'{e}matiques.}}

% Authors: full names plus addresses.
\author{
  Andy T. S. Wan\thanks{Department of Mathematics and Statistics, McGill University, Montr\'eal, QC, H3A 0B9, Canada
    (\email{andy.wan@mcgill.ca}).}
    \and
  Jean-Christophe Nave\thanks{Department of Mathematics and Statistics, McGill University, Montr\'eal,  QC, H3A 0B9, Canada (\email{jcnave@math.mcgill.ca}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

\usepackage{amstext,amsmath,amssymb}
\usepackage{enumerate}
\newtheorem{example}{Example}
\newsiamthm{claim}{Claim}
\newsiamthm{remark}{Remark}
\newsiamthm{hypo}{Hypothesis}

\def\[#1\]{\begin{align*}#1\end{align*}}

\providecommand{\pair}[1]{\langle#1\rangle}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\cont[1]{[#1]}
\newcommand\disc[1]{\{#1\}}
\newcommand\contdep[2]{[#1]_{#2}}
\newcommand\discdep[2]{\{#1\}_{#2}}
\newcommand\mesh{\mathcal{I}^\tau\times\Omega^h}
\newcommand\tmesh{\mathcal{I}^\tau}
\newcommand{\bb}{\boldsymbol }
%\newcommand\cm[1]{\mathcal{EA}_#1}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

